Improvement-Focused Causal Recourse (ICR)

Algorithmic recourse recommendations, such as Karimi et al.'s (2021) causal recourse (CR), inform stakeholders of how to act to revert unfavourable decisions. However, some actions lead to acceptance (i.e., revert the model's decision) but do not lead to improvement (i.e., may not revert the underlying real-world state). To recommend such actions is to recommend fooling the predictor. We introduce a novel method, Improvement-Focused Causal Recourse (ICR), which involves a conceptual shift: Firstly, we require ICR recommendations to guide towards improvement. Secondly, we do not tailor the recommendations to be accepted by a specific predictor. Instead, we leverage causal knowledge to design decision systems that predict accurately pre- and post-recourse. As a result, improvement guarantees translate into acceptance guarantees. We demonstrate that given correct causal knowledge, ICR, in contrast to existing approaches, guides towards both acceptance and improvement.

==> experiment-figure-option1.tex <==
\begin{figure*}[t]
\centering
\subcaptionbox{observed improvement rates $\gamma^{obs}$ (Q1)\label{subfig:improvement}}[0.38\textwidth]{
    \centering
  \includegraphics[width=.99\linewidth]{neurips-2022/figures/summary_improvement.pdf}
  
}
\hfill
\subcaptionbox{causal graphs\label{subfig:graphs}}[0.20\textwidth]{
\centering
  \begin{tikzpicture}[thick, scale=.3, every node/.style={scale=.65, line width=0.25mm, black, fill=white}]
    \usetikzlibrary{shapes}
    
        \node[fill=RoyalBlue, ellipse, scale=0.9] (a1) at (-4, 2) {};
        \node[fill=RoyalBlue, ellipse, scale=0.9] (a2) at (-1, 2) {};
        \node[fill=RoyalBlue, ellipse, scale=0.9] (a3) at (-2.5, 1) {};
        \node[fill=black, ellipse, scale=0.9] (ay) at (-2.5, -0.5) {};
        
        \draw[-stealth, gray, scale=0.3] (a1) -- (a2);
        \draw[-stealth, gray, scale=0.3] (a1) -- (a3);
        \draw[-stealth, gray, scale=0.3] (a1) -- (ay);
        \draw[-stealth, gray, scale=0.3] (a2) -- (a3);
        \draw[-stealth, gray, scale=0.3] (a2) -- (ay);
        \draw[-stealth, gray, scale=0.3] (a3) -- (ay);
        
        
        \node[fill=orange, ellipse, scale=0.9] (b1) at (3, 2) {};
        \node[fill=orange, ellipse, scale=0.9] (b2) at (0, 2) {};
        \node[fill=black, ellipse, scale=0.9] (b3) at (1.5, 1) {};
        \node[fill=orange, ellipse, scale=0.9] (by) at (1.5, -0.5) {};
        
        \draw[-stealth, gray, scale=0.3] (b1) -- (b2);
        \draw[-stealth, gray, scale=0.3] (b1) -- (b3);
        \draw[-stealth, gray, scale=0.3] (b1) -- (by);
        \draw[-stealth, gray, scale=0.3] (b2) -- (b3);
        \draw[-stealth, gray, scale=0.3] (b2) -- (by);
        \draw[-stealth, gray, scale=0.3] (b3) -- (by);
        
        \node[fill=Green, ellipse, scale=0.9] (c1) at (3, -3) {};
        \node[fill=Green, ellipse, scale=0.9] (c2) at (2, -3) {};
        \node[fill=Green, ellipse, scale=0.9] (c3) at (1, -3) {};
        \node[fill=Green, ellipse, scale=0.9] (c4) at (2, -3) {};
        \node[fill=black, ellipse, scale=0.9] (cy) at (1.5, -4.5) {};
        \node[fill=Green, ellipse, scale=0.9] (c5) at (2.5, -6) {};
        \node[fill=Green, ellipse, scale=0.9] (c6) at (1.5, -6) {};
        \node[fill=Green, ellipse, scale=0.9] (c7) at (0.5, -6) {};
        
        \draw[-stealth, gray, scale=0.3] (c1) -- (cy);
        \draw[-stealth, gray, scale=0.3] (c2) -- (cy);
        \draw[-stealth, gray, scale=0.3] (c3) -- (cy);
        \draw[-stealth, gray, scale=0.3] (c4) -- (cy);
        \draw[-stealth, gray, scale=0.3] (c1) -- (c5);
        \draw[-stealth, gray, scale=0.3] (cy) -- (c5);
        \draw[-stealth, gray, scale=0.3] (cy) -- (c6);
        \draw[-stealth, gray, scale=0.3] (cy) -- (c7);
        
        
        \node[fill=red, ellipse, scale=0.9] (d1) at (-3.5, -3) {};
        \node[fill=red, ellipse, scale=0.9] (d2) at (-1.5, -3) {};
        \node[fill=black, ellipse, scale=0.9] (dy) at (-2.5, -4.5) {};
        \node[fill=red, ellipse, scale=0.9] (d3) at (-4, -6) {};
        \node[fill=red, ellipse, scale=0.9] (d4) at (-2.5, -6) {};
        \node[fill=red, ellipse, scale=0.9] (d5) at (-1, -6) {};
        
        \draw[-stealth, gray, scale=0.3] (d1) -- (dy);
        \draw[-stealth, gray, scale=0.3] (d2) -- (dy);
        \draw[-stealth, gray, scale=0.3] (dy) -- (d3);
        \draw[-stealth, gray, scale=0.3] (dy) -- (d4);
        \draw[-stealth, gray, scale=0.3] (dy) -- (d5);
        \draw[-stealth, gray, scale=0.3] (d1) -- (d3);
    \end{tikzpicture}
  \vspace{0.5cm}
}
\hfill
\subcaptionbox{recourse cost (Q4)}[0.3\textwidth]{
\centering
\input{neurips-2022/table-cost}
\vspace{0.5cm}
}

\bigskip
%\hfill
\subcaptionbox{obs. acceptance rates $\eta^{obs}$ w.r.t. $h^*$; for ind. ICR additionally w.r.t. $h^{*,ind}$ (Q2)\label{subfig:acceptance}}[0.38\textwidth]{
%\begin{subfigure}{0.43\textwidth}
  %\centering
  \includegraphics[width=.99\linewidth]{neurips-2022/figures/summary_acceptance.pdf}
 % \caption{observed acceptance rates $\eta^{obs}$ w.r.t. the pre-recourse predictor, for ind. ICR additionally w.r.t. the ind. post-recourse predictor (squared markers) (Q2)}
%\end{subfigure}
}
\hfill
\subcaptionbox{observed acceptance rates for other fits with comparable test set performance $\eta^{obs, \text{refit}}$ (Q3)\label{subfig:acceptance-refits}}[0.38\textwidth]{
%\begin{subfigure}{0.43\textwidth}
  %\centering
  \includegraphics[width=.99\linewidth]{neurips-2022/figures/summary_acceptance_refit.pdf}
  %\caption{observed acceptance rates for other fits on the same data with comparable test set performance $\eta^{obs, \text{refit}}$ (Q3)}
%\end{subfigure}
}
\hfill
\subcaptionbox{legend\label{subfig:legend}}[0.15\textwidth]{
%\begin{subfigure}{0.12\textwidth}
  %\subcaptionbox{legend}[0.2\textwidth]{
    \centering
  \includegraphics[width=.99\linewidth]{neurips-2022/figures/legend.pdf}
 % \caption{legend}
  %\vspace{0.3cm}
%}
%\end{subfigure}
}
%\hfill
\caption{%Observed improvement rate $\gamma^{obs}$, acceptance rate $\eta^{obs}$, mean acceptance rate on five refits $\eta^{obs, refit}$, and cost of individuals implementing CE, CR and ICR recommendations on 3var-causal (blue), 3var-noncausal (orange), 7var-covid (green). 
Experimental results for CE, CR and ICR on four datasets over $10$ runs on $200$ individuals each.
For the probabilistic methods the confidences $0.75, 0.85, 0.9, 0.95$ were targeted (for CR: $\overline{\eta}$, for ICR: $\overline{\gamma}$). For CE no slack is allowed, such that the results correspond to a confidence level of $1.0$. Values are reported on a quadratic scale.}
\label{fig:experiment-results}
\end{figure*}

==> figures/causal-graphs.tex <==
\begin{tikzpicture}[thick, scale=.23, every node/.style={scale=.6, line width=0.25mm, black, fill=white}]
    \usetikzlibrary{shapes}
        \node[fill=RoyalBlue, ellipse, scale=0.9] (a1) at (-4, 2) {};
        \node[fill=RoyalBlue, ellipse, scale=0.9] (a2) at (-1, 2) {};
        \node[fill=RoyalBlue, ellipse, scale=0.9] (a3) at (-2.5, 1) {};
        \node[fill=black, ellipse, scale=0.9] (ay) at (-2.5, -0.5) {};
        
        \draw[-stealth, gray, scale=0.3] (a1) -- (a2);
        \draw[-stealth, gray, scale=0.3] (a1) -- (a3);
        \draw[-stealth, gray, scale=0.3] (a1) -- (ay);
        \draw[-stealth, gray, scale=0.3] (a2) -- (a3);
        \draw[-stealth, gray, scale=0.3] (a2) -- (ay);
        \draw[-stealth, gray, scale=0.3] (a3) -- (ay);
        
        
        \node[fill=orange, ellipse, scale=0.9] (b1) at (3, 2) {};
        \node[fill=orange, ellipse, scale=0.9] (b2) at (0, 2) {};
        \node[fill=black, ellipse, scale=0.9] (b3) at (1.5, 1) {};
        \node[fill=orange, ellipse, scale=0.9] (by) at (1.5, -0.5) {};
        
        \draw[-stealth, gray, scale=0.3] (b1) -- (b2);
        \draw[-stealth, gray, scale=0.3] (b1) -- (b3);
        \draw[-stealth, gray, scale=0.3] (b1) -- (by);
        \draw[-stealth, gray, scale=0.3] (b2) -- (b3);
        \draw[-stealth, gray, scale=0.3] (b2) -- (by);
        \draw[-stealth, gray, scale=0.3] (b3) -- (by);
        
        \node[fill=Green, ellipse, scale=0.9] (c1) at (3, -3) {};
        \node[fill=Green, ellipse, scale=0.9] (c2) at (2, -3) {};
        \node[fill=Green, ellipse, scale=0.9] (c3) at (1, -3) {};
        \node[fill=Green, ellipse, scale=0.9] (c4) at (2, -3) {};
        \node[fill=black, ellipse, scale=0.9] (cy) at (1.5, -4.5) {};
        \node[fill=Green, ellipse, scale=0.9] (c5) at (2.5, -6) {};
        \node[fill=Green, ellipse, scale=0.9] (c6) at (1.5, -6) {};
        \node[fill=Green, ellipse, scale=0.9] (c7) at (0.5, -6) {};
        
        \draw[-stealth, gray, scale=0.3] (c1) -- (cy);
        \draw[-stealth, gray, scale=0.3] (c2) -- (cy);
        \draw[-stealth, gray, scale=0.3] (c3) -- (cy);
        \draw[-stealth, gray, scale=0.3] (c4) -- (cy);
        \draw[-stealth, gray, scale=0.3] (c1) -- (c5);
        \draw[-stealth, gray, scale=0.3] (cy) -- (c5);
        \draw[-stealth, gray, scale=0.3] (cy) -- (c6);
        \draw[-stealth, gray, scale=0.3] (cy) -- (c7);
        
        
        \node[fill=red, ellipse, scale=0.9] (d1) at (-3.5, -3) {};
        \node[fill=red, ellipse, scale=0.9] (d2) at (-1.5, -3) {};
        \node[fill=black, ellipse, scale=0.9] (dy) at (-2.5, -4.5) {};
        \node[fill=red, ellipse, scale=0.9] (d3) at (-4, -6) {};
        \node[fill=red, ellipse, scale=0.9] (d4) at (-2.5, -6) {};
        \node[fill=red, ellipse, scale=0.9] (d5) at (-1, -6) {};
        
        \draw[-stealth, gray, scale=0.3] (d1) -- (dy);
        \draw[-stealth, gray, scale=0.3] (d2) -- (dy);
        \draw[-stealth, gray, scale=0.3] (dy) -- (d3);
        \draw[-stealth, gray, scale=0.3] (dy) -- (d4);
        \draw[-stealth, gray, scale=0.3] (dy) -- (d5);
        \draw[-stealth, gray, scale=0.3] (d1) -- (d3);
    \end{tikzpicture}

==> latex-math/ml-automl.tex <==


% lambdav
\newcommand{\lambdav}{\bm{\lambda}}											% lambda vector



==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(x)}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(x)}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(x)}                    % ensembled predictor
\newcommand{\fMh}{\hat f^{[M]}(x)}                    % estimated ensembled predictor
\newcommand{\ambifM}{\Delta\left(\fM\right)}          % ambiguity/instability of ensemble


==> latex-math/ml-bayesopt.tex <==
% ml - Bayesian Optimization

\newcommand{\minit}{m_{\text{init}}											% Size of the initial design
\newcommand{\lambdai}{\lambda^{[i]}											% input for black box optimization 
\newcommand{\lambdaopt}{\lambda^{*}}											% Minimum of the black box function Psi
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\left(\lambda^{[1]}, \dots, \lambda^{[\minit]}\right)}  % Vector of different inputs


% \newcommand{\metadata}



\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process 


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{r^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{r^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}

==> latex-math/ml-feature-sel.tex <==
% ml - feature selection

\newcommand{\xjNull}{x_{j_0}}
\newcommand{\xjEins}{x_{j_1}}
\newcommand{\xl}{\mathbf{x}_l}
\newcommand{\pushcode}[1][1]{\hskip\dimexpr#1\algorithmicindent\relax}

==> latex-math/ml-gp.tex <==
% ml - Gaussian Process

\newcommand{\gp}{\mathcal{GP}\left(m(\bm{x}), k\left(\bm{x}, \bm{x}^\prime\right)\right)} 								% Gaussian Process Definition	
\newcommand{\mvec}{\mathbf{m}}												    						% Gaussian process mean vector
\newcommand{\Kmat}{\mathbf{K}}																			% estimated base learner 
\newcommand{\ls}{\ell}                                           % length-scale


==> latex-math/ml-lm.tex <==
\newcommand{\thx}{\thetab^T \xv}												% linear score: theta^T x



==> latex-math/ml-mbo.tex <==
% ml - MBO
\newcommand{\sxh}{\hat{s}(x)} % uncertainty shat(x)
\newcommand{\vxh}{\hat{s}^2(x)}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\kstarx}{\mathbf{k}_*(x)}
\newcommand{\xpi}[1][i]{x^{*(#1)}}
\newcommand{\vhx}{\ensuremath{\sh^2(\xv)}\xspace}          % local estimated variance at point x
\newcommand{\shx}{\ensuremath{\sh(\xv)}\xspace}            % local estimated uncertainty at point x
\newcommand{\sh}{\ensuremath{\hat{s}}\xspace}              % local estimated uncertainty
\newcommand{\px}{\ensuremath{\boldsymbol{x}^*}}
\newcommand{\equote}[1]{``#1''}
\newcommand{\vecx}{\ensuremath{\boldsymbol{x}}}
\newcommand{\yx}{\ensuremath{y(\vecx)}}
\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace}           % domain / search space

% already defined in basic-math:
% \newcommand{\yv}{\boldsymbol{y}}
\newcommand{\fhx}{\ensuremath{\fh(\xv)}\xspace}            % surrogate (x), better use \mhx for predicted value



\newcommand{\minit}{m_{\text{init}}}											% Size of the initial design
\newcommand{\lambdai}{\lambdab^{[i]}}											% input for black box optimization 
\newcommand{\lambdanew}{\lambdab^{\text{new}}}								% new proposed configuration
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\lambdab^{[1]}, ..., \lambdab^{[\minit]}}  % Vector of different inputs
\newcommand{\lambdab}{\boldsymbol{\lambda}}									% input 
\newcommand{\lambdaopt}{\lambdab^{*}}											% Minimum of the black box function Psi


==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector

\newcommand{\biasc}{c}                          % bias in output


\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)

\newcommand{\Wmat}{\mathbf{W}}                             % weight vector (general)


\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Loss}{L(y, f(\xv, \thetab))}
\newcommand{\Lmomentumnest}{L(\yi, f(x^{(i)}, \thetab + \varphi \nub))}                  % momentum risk
\newcommand{\Lmomentumtilde}{L(\yi, f(x^{(i)}, \tilde{\thetab}))}                  % Nesterov momentum risk
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \thetab))} 
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\nub}{\boldsymbol{\nu}}

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function

% deeplearning - adversarials 
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\Lossdeltai}{L(\yi, f(\xi + \deltab|\thetab))}
\newcommand{\Lossdelta}{L(y, f(\xv + \deltab| \thetab))}

==> latex-math/ml-rf.tex <==
% ml -  ensemble methods, random forest

\newcommand{\betam}{\beta^{[m]}}												% baselearner with argument for m
\newcommand{\betaM}{\beta^{[M]}}												% baselearner with argument for M
\newcommand{\betai}{\beta^{[1]}}												% baselearner with argument for 1


==> latex-math/ml-survival.tex <==
\newcommand{\Ti}[1][i]{T^{(#1)}}
\newcommand{\Ci}[1][i]{C^{(#1)}}  
\newcommand{\oi}[1][i]{o^{(#1)}}  
\newcommand{\ti}[1][i]{t^{(#1)}}  
\newcommand{\lambdai}[1][i]{\lambda^{(#1)}}  
\newcommand{\deltai}[1][i]{\delta^{(#1)}}  
\newcommand{\Lxdi}{L\left(\bm{\delta}, \fx\right)}           



==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
% \newcommand{\HS}{\mathcal{H}}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Npk}{\Np_k}														% node N_k
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\pi_k^{(\Np)}}                                           		% class probability node N
\newcommand{\pikNh}[1][k]{\hat\pi_#1^{(\Np)}}                                           % estimated class probability node N
\newcommand{\pikNlh}[1][k]{\hat\pi_#1^{(\Nl)}}
\newcommand{\pikNrh}[1][k]{\hat\pi_#1^{(\Nr)}}

==> latex-math/probmodel.tex <==


% gaussians
\newcommand{\muk}{\bm{\mu_k}}  


==> legacy/figures_results.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.2\linewidth}
      \input{arxiv-preprint/figures/causal-graphs}
    \end{subfigure}
    \hspace{0.7cm}
    \hfill
    \begin{subfigure}{0.33\linewidth}
      \includegraphics[width=.99\linewidth]{arxiv-preprint/figures/legend_scm}
      \vspace{0.1cm}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.33\linewidth}
      \includegraphics[width=.99\linewidth]{arxiv-preprint/figures/legend_type}
      \vspace{0.5cm}
    \end{subfigure}
    \caption{Left: Causal graphs. Right: Legend for color (SCM) and linestyle (recourse type) in Figures \ref{fig:improvement-rates}, \ref{fig:acceptance-rates} and \ref{fig:acceptance-rates-refits}.}
    \label{fig:legend}
\end{figure}
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{arxiv-preprint/figures/summary_improvement.pdf}
    \caption{Observed improvement rates $\gamma^{obs}$ (Q1).}
    \label{fig:improvement-rates}
\end{figure}
%
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{arxiv-preprint/figures/summary_acceptance.pdf}
    \caption{Observed acceptance rates $\eta^{obs}$ w.r.t. $h^*$; for ind. ICR additionally w.r.t. $h^{*,ind}$ (Q2).}
    \label{fig:acceptance-rates}
\end{figure}
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{arxiv-preprint/figures/summary_acceptance_refit.pdf}
    \caption{Observed acceptance rates for other fits with comparable test set performance $\eta^{obs, \text{refit}}$ (Q3).}
    \label{fig:acceptance-rates-refits}
\end{figure}
%
\begin{table}[b]
    \centering
    \caption{Recourse cost (Q4).}
    \include{arxiv-preprint/table-cost}
    \label{table:cost}
\end{table}

==> notation.tex <==
%\usepackage{pxfonts}
%\usepackage{mathtools}

\newcommand{\approxd}{\stackrel{\mathclap{\normalfont\mbox{$d$}}}{\approx}} % equality in distribution
\newcommand{\eqd}{\stackrel{\mathclap{\normalfont\mbox{$d$}}}{=}} % equality in distribution

\newcommand{\fimp}{\text{FI}}
\newcommand{\rfi}{\text{RFI}}
\newcommand{\rfijg}{\rfi_j^G}
\newcommand{\rfijgn}{\rfi_j^{G \cup N}}
\newcommand{\deltarfi}{\Delta RFI_j^{G \to G \cup N}}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\risktj}{\tilde{\risk}^j}
\newcommand{\risktjg}{\tilde{\risk}^{j|G}}

\newcommand{\Ru}{\underline{R}}
\newcommand{\Ruu}{\underline{\underline{R}}}
\newcommand{\Go}{\overline{G}}
\newcommand{\No}{\overline{N}}
\newcommand{\Gs}{G^*}
\newcommand{\Ns}{N^*}
\newcommand{\Du}{\underline{D}}

\newcommand{\uX}{\underline{X}}
\newcommand{\tXjg}{\tilde{X}_j^G}
\newcommand{\tXjgn}{\tilde{X}_j^{G \cup N}}
\newcommand{\XR}{X_R}
\newcommand{\XRu}{X_{\Ru}}
\newcommand{\XRuu}{X_{\Ruu}}
\newcommand{\XG}{X_G}
\newcommand{\XGs}{X_\Gs}
\newcommand{\XNs}{X_\Ns}
\newcommand{\Xj}{X_j}
\newcommand{\Yh}{\hat{Y}}
% yhat already defined in latex-maths
%\newcommand{\yh}{\hat{y}}

\newcommand{\idp}{\perp}
\newcommand{\dpd}{\not \idp}
